Causal Order Discovery based on Monotonic SCMs

In this paper, we consider the problem of causal order discovery within the framework of monotonic Structural Causal Models (SCMs), which have gained attention for their potential to enable causal inference and causal discovery from observational data. While existing approaches either assume prior knowledge about the causal order or use complex optimization techniques to impose sparsity in the Jacobian of Triangular Monotonic Increasing maps, our work introduces a novel sequential procedure that directly identifies the causal order by iteratively detecting the root variable. This method eliminates the need for sparsity assumptions and the associated optimization challenges, enabling the identification of a unique SCM without the need for multiple independence tests to break the Markov equivalence class. We demonstrate the effectiveness of our approach in sequentially finding the root variable, comparing it to methods that maximize Jacobian sparsity.

==> Styles/refs.tex <==
@BOOK{Scholkopf2017-da,
  title     = "Elements of causal inference: Foundations and learning
               algorithms",
  author    = "Scholkopf, Bernhard and Peters, Jonas and Janzing, Dominik",
  publisher = "MIT Press",
  year      =  2017,
}   

@article{zanga2022survey,
  title={A survey on causal discovery: theory and practice},
  author={Zanga, Alessio and Ozkirimli, Elif and Stella, Fabio},
  journal={International Journal of Approximate Reasoning},
  volume={151},
  pages={101--129},
  year={2022},
  publisher={Elsevier}
}


@article{imbens2004nonparametric,
  title={Nonparametric estimation of average treatment effects under exogeneity: A review},
  author={Imbens, Guido W},
  journal={Review of Economics and statistics},
  volume={86},
  number={1},
  pages={4--29},
  year={2004},
  publisher={MIT Press 238 Main St., Suite 500, Cambridge, MA 02142-1046, USA journals~…}
}

@article{glymour2019review,
  title={Review of causal discovery methods based on graphical models},
  author={Glymour, Clark and Zhang, Kun and Spirtes, Peter},
  journal={Frontiers in genetics},
  volume={10},
  pages={524},
  year={2019},
  publisher={Frontiers Media SA}
}



@article{malinsky2018causal,
  title={Causal discovery algorithms: A practical guide},
  author={Malinsky, Daniel and Danks, David},
  journal={Philosophy Compass},
  volume={13},
  number={1},
  pages={e12470},
  year={2018},
  publisher={Wiley Online Library}
}


@article{kaddour2022causal,
  title={Causal machine learning: A survey and open problems},
  author={Kaddour, Jean and Lynch, Aengus and Liu, Qi and Kusner, Matt J and Silva, Ricardo},
  journal={arXiv preprint arXiv:2206.15475},
  year={2022}
}


@BOOK{pearl2009causality,
  title     = "Causality: Models, reasoning, and inference",
  author    = "Pearl, Judea",
  publisher = "Cambridge University Press",
  year      =  2009,
}

@article{shimizu2006linear,
  title={A linear non-Gaussian acyclic model for causal discovery.},
  author={Shimizu, Shohei and Hoyer, Patrik O and Hyv{\"a}rinen, Aapo and Kerminen, Antti and Jordan, Michael},
  journal={Journal of Machine Learning Research},
  volume={7},
  number={10},
  year={2006}
}

@article{hoyer2008nonlinear,
  title={Nonlinear causal discovery with additive noise models},
  author={Hoyer, Patrik and Janzing, Dominik and Mooij, Joris M and Peters, Jonas and Sch{\"o}lkopf, Bernhard},
  journal={Advances in neural information processing systems},
  volume={21},
  year={2008}
}

@inproceedings{10.5555/1795114.1795190,
author = {Zhang, Kun and Hyv\"{a}rinen, Aapo},
title = {On the Identifiability of the Post-Nonlinear Causal Model},
year = {2009},
booktitle = {Proceedings of the Twenty-Fifth Conference on Uncertainty in Artificial Intelligence},
publisher = {AUAI Press},
pages = {647–655},
volume = {9},
}

@inproceedings{xi2023indeterminacy,
  title={Indeterminacy in generative models: Characterization and strong identifiability},
  author={Xi, Quanhan and Bloem-Reddy, Benjamin},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={6912--6939},
  year={2023},
  organization={PMLR}
}


@inproceedings{rezende2015variational,
  title={Variational inference with normalizing flows},
  author={Rezende, Danilo and Mohamed, Shakir},
  booktitle={International conference on machine learning},
  pages={1530--1538},
  year={2015},
  organization={PMLR}
}


@article{javaloy2024causal,
  title={Causal normalizing flows: from theory to practice},
  author={Javaloy, Adri{\'a}n and S{\'a}nchez-Mart{\'\i}n, Pablo and Valera, Isabel},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@inproceedings{xi2023triangular,
  title={Triangular monotonic generative models can perform causal discovery},
  author={Xi, Quanhan and Gonzalez, Sebastian and Bloem-Reddy, Benjamin},
  booktitle={Causal Representation Learning Workshop at NeurIPS 2023},
  year={2023}
}


@inproceedings{khemakhem2021causal,
  title={Causal autoregressive flows},
  author={Khemakhem, Ilyes and Monti, Ricardo and Leech, Robert and Hyvarinen, Aapo},
  booktitle={International conference on artificial intelligence and statistics},
  pages={3520--3528},
  year={2021},
  organization={PMLR}
}


@article{hyvarinen2024identifiability,
  title={Identifiability of latent-variable and structural-equation models: from linear to nonlinear},
  author={Hyv{\"a}rinen, Aapo and Khemakhem, Ilyes and Monti, Ricardo},
  journal={Annals of the Institute of Statistical Mathematics},
  volume={76},
  number={1},
  pages={1--33},
  year={2024},
  publisher={Springer}
}


@inproceedings{monti2020causal,
  title={Causal discovery with general non-linear relationships using non-linear ica},
  author={Monti, Ricardo Pio and Zhang, Kun and Hyv{\"a}rinen, Aapo},
  booktitle={Uncertainty in artificial intelligence},
  pages={186--195},
  year={2020},
  organization={PMLR}
}

@article{reizinger2023jacobian,
  title={Jacobian-based causal discovery with nonlinear ICA},
  author={Reizinger, Patrik and Sharma, Yash and Bethge, Matthias and Sch{\"o}lkopf, Bernhard and Husz{\'a}r, Ferenc and Brendel, Wieland},
  journal={Transactions on Machine Learning Research},
  year={2023}
}

@article{mena2018learning,
  title={Learning latent permutations with gumbel-sinkhorn networks},
  author={Mena, Gonzalo and Belanger, David and Linderman, Scott and Snoek, Jasper},
  journal={arXiv preprint arXiv:1802.08665},
  year={2018}
}


@inproceedings{rolland2022score,
  title={Score matching enables causal discovery of nonlinear additive noise models},
  author={Rolland, Paul and Cevher, Volkan and Kleindessner, Matth{\"a}us and Russell, Chris and Janzing, Dominik and Sch{\"o}lkopf, Bernhard and Locatello, Francesco},
  booktitle={International Conference on Machine Learning {ICML}},
  pages={18741--18753},
  year={2022},
  organization={PMLR}
}

@article{reisach2021beware,
  title={Beware of the simulated dag! varsortability in additive noise models},
  author={Reisach, Alexander G and Seiler, Christof and Weichwald, Sebastian},
  journal={Advances in neural information processing systems},
  volume={13},
  year={2021}
}

@article{durkan2019neural,
  title={Neural spline flows},
  author={Durkan, Conor and Bekasov, Artur and Murray, Iain and Papamakarios, George},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@ARTICLE{Sachs2005-cu,
  title    = "Causal protein-signaling networks derived from multiparameter
              single-cell data",
  author   = "Sachs, Karen and Perez, Omar and Pe'er, Dana and Lauffenburger,
              Douglas A and Nolan, Garry P",
  journal  = "Science",
  volume   =  308,
  number   =  5721,
  pages    = "523--529",
  year     =  2005,
}

@article{van2006syntren,
  title={SynTReN: a generator of synthetic gene expression data for design and analysis of structure learning algorithms},
  author={Van den Bulcke, Tim and Van Leemput, Koenraad and Naudts, Bart and van Remortel, Piet and Ma, Hongwu and Verschoren, Alain and De Moor, Bart and Marchal, Kathleen},
  journal={BMC bioinformatics},
  volume={7},
  pages={1--12},
  year={2006},
  publisher={Springer}
}

@article{bogachev2005triangular,
  title={Triangular transformations of measures},
  author={Bogachev, Vladimir Igorevich and Kolesnikov, Aleksandr Viktorovich and Medvedev, Kirill Vladimirovich},
  journal={Sbornik: Mathematics},
  volume={196},
  number={3},
  pages={309},
  year={2005},
  publisher={IOP Publishing}
}

@article{carlier2010knothe,
  title={From Knothe's transport to Brenier's map and a continuation method for optimal transport},
  author={Carlier, Guillaume and Galichon, Alfred and Santambrogio, Filippo},
  journal={SIAM Journal on Mathematical Analysis},
  volume={41},
  number={6},
  pages={2554--2576},
  year={2010},
  publisher={SIAM}
}

@article{papamakarios2021normalizing,
  title={Normalizing flows for probabilistic modeling and inference},
  author={Papamakarios, George and Nalisnick, Eric and Rezende, Danilo Jimenez and Mohamed, Shakir and Lakshminarayanan, Balaji},
  journal={The Journal of Machine Learning Research},
  volume={22},
  number={1},
  pages={2617--2680},
  year={2021},
  publisher={JMLRORG}
}

@inproceedings{irons2022triangular,
  title={Triangular flows for generative modeling: Statistical consistency, smoothness classes, and fast rates},
  author={Irons, Nicholas J and Scetbon, Meyer and Pal, Soumik and Harchaoui, Zaid},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={10161--10195},
  year={2022},
  organization={PMLR}
}

@article{hotelling1931generalization,
  title={The generalization of Student's ratio},
  author={Hotelling, Harold and others},
  year={1931},
  publisher={Springer}
}

@article{peters2014causal,
  author  = {Jonas Peters and Joris M. Mooij and Dominik Janzing and Bernhard Sch{{\"o}}lkopf},
  title   = {Causal Discovery with Continuous Additive Noise Models},
  journal = {Journal of Machine Learning Research {JMLR}},
  year    = {2014},
  volume  = {15},
  number  = {58},
  pages   = {2009--2053},
}

@article{buhlmann2014cam,
author = {Peter B{\"u}hlmann and Jonas Peters and Jan Ernest},
title = {{CAM: Causal additive models, high-dimensional order search and penalized regression}},
volume = {42},
journal = {The Annals of Statistics},
number = {6},
publisher = {Institute of Mathematical Statistics},
pages = {2526 -- 2556},
year = {2014},
}

@article{wang2021ordering,
  title={Ordering-based causal discovery with reinforcement learning},
  author={Wang, Xiaoqiang and Du, Yali and Zhu, Shengyu and Ke, Liangjun and Chen, Zhitang and Hao, Jianye and Wang, Jun},
  journal={arXiv preprint arXiv:2105.06631},
  year={2021}
}

@article{raskutti2018learning,
  title={Learning directed acyclic graph models based on sparsest permutations},
  author={Raskutti, Garvesh and Uhler, Caroline},
  journal={Stat},
  volume={7},
  number={1},
  pages={e183},
  year={2018},
  publisher={Wiley Online Library}
}

@article{squires2020efficient,
  title={Efficient Permutation Discovery in Causal DAGs},
  author={Squires, Chandler and Amaniampong, Joshua and Uhler, Caroline},
  journal={arXiv preprint arXiv:2011.03610},
  year={2020}
}

@article{charpentier2022differentiable,
  title={Differentiable DAG sampling},
  author={Charpentier, Bertrand and Kibler, Simon and G{\"u}nnemann, Stephan},
  journal={arXiv preprint arXiv:2203.08509},
  year={2022}
}

@article{zantedeschi2023dag,
  title={DAG Learning on the Permutahedron},
  author={Zantedeschi, Valentina and Franceschi, Luca and Kaddour, Jean and Kusner, Matt J and Niculae, Vlad},
  journal={arXiv preprint arXiv:2301.11898},
  year={2023}
}

@article{cundy2021bcd,
  title={Bcd nets: Scalable variational approaches for bayesian causal discovery},
  author={Cundy, Chris and Grover, Aditya and Ermon, Stefano},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={7095--7110},
  year={2021}
}


@article{sanchez2022diffusion,
  title={Diffusion Models for Causal Discovery via Topological Ordering},
  author={Sanchez, Pedro and Liu, Xiao and O'Neil, Alison Q and Tsaftaris, Sotirios A},
  journal={arXiv preprint arXiv:2210.06201},
  year={2022}
}


@article{montagna2023causal,
  title={Causal Discovery with Score Matching on Additive Models with Arbitrary Noise},
  author={Montagna, Francesco and Noceti, Nicoletta and Rosasco, Lorenzo and Zhang, Kun and Locatello, Francesco},
  journal={arXiv preprint arXiv:2304.03265},
  year={2023}
}

@InProceedings{montagna2023scalable,
  title = 	 {Scalable Causal Discovery with Score Matching},
  author =       {Montagna, Francesco and Noceti, Nicoletta and Rosasco, Lorenzo and Zhang, Kun and Locatello, Francesco},
  booktitle = 	 {Proceedings of the Second Conference on Causal Learning and Reasoning},
  pages = 	 {752--771},
  year = 	 {2023},
  volume = 	 {213},
  publisher =    {PMLR}
}

@article{zhu2024sample,
  title={Sample complexity bounds for score-matching: causal discovery and generative modeling},
  author={Zhu, Zhenyu and Locatello, Francesco and Cevher, Volkan},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}


@inproceedings{uemura2022multivariate,
  title={A multivariate causal discovery based on post-nonlinear model},
  author={Uemura, Kento and Takagi, Takuya and Takayuki, Kambayashi and Yoshida, Hiroyuki and Shimizu, Shohei},
  booktitle={Conference on Causal Learning and Reasoning},
  pages={826--839},
  year={2022},
  organization={PMLR}
}

@inproceedings{keropyan2023rank,
  title={Rank-Based Causal Discovery for Post-Nonlinear Models},
  author={Keropyan, Grigor and Strieder, David and Drton, Mathias},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={7849--7870},
  year={2023},
  organization={PMLR}
}

@inproceedings{
akbari2023causal,
title={Causal Discovery via Monotone Triangular Transport Maps},
author={Sina Akbari and Luca Ganassali and Negar Kiyavash},
booktitle={NeurIPS 2023 Workshop Optimal Transport and Machine Learning},
year={2023},
url={https://openreview.net/forum?id=PMGGrKTIii}
}

@inproceedings{nasr2023counterfactual,
  title={Counterfactual identifiability of bijective causal models},
  author={Nasr-Esfahany, Arash and Alizadeh, Mohammad and Shah, Devavrat},
  booktitle={International Conference on Machine Learning},
  pages={25733--25754},
  year={2023},
  organization={PMLR}
}

@inproceedings{scetbonfixed,
  title={A Fixed-Point Approach for Causal Generative Modeling},
  author={Scetbon, Meyer and Jennings, Joel and Hilmkil, Agrin and Zhang, Cheng and Ma, Chao},
  booktitle={Forty-first International Conference on Machine Learning},
  year={2024}
}


@article{kamkari2023ocdaf,
  title={Ocdaf: Ordered causal discovery with autoregressive flows},
  author={Kamkari, Hamidreza and Zehtab, Vahid and Balazadeh, Vahid and Krishnan, Rahul G},
  journal={arXiv preprint arXiv:2308.07480},
  year={2023}
}

@book{spirtes2001causation,
  title={Causation, prediction, and search},
  author={Spirtes, Peter and Glymour, Clark and Scheines, Richard},
  year={2001},
  publisher={MIT press}
}

@article{shimizu2011directlingam,
  title={DirectLiNGAM: A direct method for learning a linear non-Gaussian structural equation model},
  author={Shimizu, Shohei and Inazumi, Takanori and Sogawa, Yasuhiro and Hyvarinen, Aapo and Kawahara, Yoshinobu and Washio, Takashi and Hoyer, Patrik O and Bollen, Kenneth and Hoyer, Patrik},
  journal={Journal of Machine Learning Research-JMLR},
  volume={12},
  number={Apr},
  pages={1225--1248},
  year={2011}
}

@article{kuhn1955hungarian,
  title={The Hungarian method for the assignment problem},
  author={Kuhn, Harold W},
  journal={Naval research logistics quarterly},
  volume={2},
  number={1-2},
  pages={83--97},
  year={1955},
  publisher={Wiley Online Library}
}

@article{spantini2018inference,
  title={Inference via low-dimensional couplings},
  author={Spantini, Alessio and Bigoni, Daniele and Marzouk, Youssef},
  journal={Journal of Machine Learning Research},
  volume={19},
  number={66},
  pages={1--71},
  year={2018}
}

@article{morrison2017beyond,
  title={Beyond normality: Learning sparse probabilistic graphical models in the non-Gaussian setting},
  author={Morrison, Rebecca and Baptista, Ricardo and Marzouk, Youssef},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{baptista2024learning,
  title={Learning non-Gaussian graphical models via Hessian scores and triangular transport},
  author={Baptista, Ricardo and Morrison, Rebecca and Zahm, Olivier and Marzouk, Youssef},
  journal={Journal of Machine Learning Research},
  volume={25},
  number={85},
  pages={1--46},
  year={2024}
}

@inproceedings{zheng2020learning,
  title={Learning sparse nonparametric dags},
  author={Zheng, Xun and Dan, Chen and Aragam, Bryon and Ravikumar, Pradeep and Xing, Eric},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3414--3425},
  year={2020},
  organization={Pmlr}
}

@inproceedings{ng2022masked,
  title={Masked gradient-based causal structure learning},
  author={Ng, Ignavier and Zhu, Shengyu and Fang, Zhuangyan and Li, Haoyang and Chen, Zhitang and Wang, Jun},
  booktitle={Proceedings of the 2022 SIAM International Conference on Data Mining (SDM)},
  pages={424--432},
  year={2022},
  organization={SIAM}
}

@inproceedings{deng2023optimizing,
  title={Optimizing NOTEARS objectives via topological swaps},
  author={Deng, Chang and Bello, Kevin and Aragam, Bryon and Ravikumar, Pradeep Kumar},
  booktitle={International Conference on Machine Learning},
  pages={7563--7595},
  year={2023},
  organization={PMLR}
}

@inproceedings{ng2024structure,
  title={Structure learning with continuous optimization: A sober look and beyond},
  author={Ng, Ignavier and Huang, Biwei and Zhang, Kun},
  booktitle={Causal Learning and Reasoning},
  pages={71--105},
  year={2024},
  organization={PMLR}
}

@article{deng2023global,
  title={Global optimality in bivariate gradient-based DAG learning},
  author={Deng, Chang and Bello, Kevin and Ravikumar, Pradeep and Aragam, Bryon},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  pages={17929--17968},
  year={2023}
}




